Implicit Training of Energy Model for Structure Prediction

Most deep learning research has focused on developing new model and training procedures. On the other hand the training objective has usually been restricted to combinations of standard losses. When the objective aligns well with the evaluation metric, this is not a major issue. However when dealing with complex structured outputs, the ideal objective can be hard to optimize and the efficacy of usual objectives as a proxy for the true objective can be questionable. In this work, we argue that the existing inference network based structure prediction methods ( Tu and Gimpel 2018; Tu, Pang, and Gimpel 2020) are indirectly learning to optimize a dynamic loss objective parameterized by the energy model. We then explore using implicit-gradient based technique to learn the corresponding dynamic objectives. Our experiments show that implicitly learning a dynamic loss landscape is an effective method for improving model performance in structure prediction.

==> header1.tex <==

% Get better typography
% \usepackage[protrusion=true,expansion=true]{microtype}		

% Small margins
%\usepackage[top=2cm, bottom=2cm, left = 1cm, right = 1cm,columnsep=20pt]{geometry}


% For basic math, align, fonts, etc.
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{bbm}
\usepackage{mathtools}
\usepackage{mathrsfs}
\usepackage{dsfont}
% \usepackage[scr=esstix,cal=boondox]{mathalfa} 

\usepackage{courier} % For \texttt{foo} to put foo in Courier (for code / variables)

\usepackage{lipsum} % For dummy text

% for underlining text

\def\mul#1#2{\color{#1}\underline{{\color{black}#2}}\color{black}}
% \usepackage{soul} 
% \newcommand{\myul}[2][black]{\setulcolor{#1}\ul{#2}\setulcolor{black}}

% For images
% \usepackage{graphicx}
% \usepackage{subcaption}
\usepackage[space]{grffile} % For spaces in image names

% For bibliography
% \usepackage[numbers]{natbib}

% For links (e.g., clicking a reference takes you to the phy)
\usepackage{hyperref}

% For color
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{xcolor}
\definecolor{dark-red}{rgb}{0.4,0.15,0.15}
\definecolor{dark-blue}{rgb}{0,0,0.7}
\hypersetup{
    colorlinks, linkcolor={dark-blue},
    citecolor={dark-blue}, urlcolor={dark-blue}
}


% Macros
\newcommand{\yash}[1]{\textcolor{blue}{[#1---yash]}}
\newcommand{\imp}[1]{\textcolor{red}{[IMP: #1]}}
\newcommand{\red}[1]{\textcolor{purple}{[#1]}}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}


% \usepackage{algpseudocode}
% \usepackage[noend,linesnumbered,ruled]{algorithm2e}
% \usepackage[vlined,linesnumbered,ruled,algo2e]{algorithm2e}
% \usepackage[vlined,ruled,algo2e]{algorithm2e}

\usepackage{algorithm}
\usepackage{algorithmic}

% \usepackage[algo2e]{algorithm2e} 
% \SetKwProg{Fn}{Function}{}{}
% \let\oldnl\nl% Store \nl in \oldnl
% \newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line

% Miscelaneous headers
\usepackage{multicol}
\usepackage{enumitem}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{bm}

\newcommand{\ind}{\perp\!\!\!\!\perp}

% Commands for organizing theorems and proofs

\usepackage{theoremref}
%\mathtoolsset{showonlyrefs}

\newtheorem{defn}{Definition}[]
\newtheorem{rem}{Remark}[]
\newtheorem{thm}{Theorem}[]
\newtheorem{claim}{Claim}[]
\newtheorem{lemma}{Lemma}[]
\newtheorem{prop}{Property}[]
\newtheorem{ass}{Assumption}[]
\newtheorem{cor}{Corollary}[]

% For creating sub-groups of Assumptions/Theorems etc.
\newtheorem{reqm}{Requirement}
% \renewcommand\thereqm{A\arabic{reqm}}

\usepackage{thmtools}
\usepackage{thm-restate}

\declaretheorem[name=Theorem]{rtheorem}
\declaretheorem[name=Proposition]{rproposition}
\declaretheorem[name=Assumption]{rassumption}
\declaretheorem[name=Corollary]{rcorollary}
\declaretheorem[name=Lemma]{rlemma}


% Definitions of handy macros can go here
\newcommand{\dataset}{{\cal D}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}
\newcommand{\pibopt}{\pi_{b^\star}}
\newcommand{\pib}{{\pi_b}}
\newcommand{\pitheta}{{\pi_\btheta}}
\newcommand{\deltheta}{{\frac{\partial}{\partial \btheta}}}
\newcommand{\delthetatwo}{{\frac{\partial^2}{\partial^2 \btheta}}}
\newcommand{\pieval}{{\pi_e}}
\newcommand{\btheta}{{\boldsymbol\theta}}
\newcommand{\data}{{\mathcal{D}}}
\newcommand{\ope}{{\operatorname{OPE}}}
\newcommand{\pe}{{\operatorname{PE}}}
\newcommand{\variance}{{\operatorname{Var}}}
\newcommand{\covariance}{{\operatorname{Cov}}}
\newcommand{\bias}{{\operatorname{Bias}}}
\newcommand{\mse}{{\operatorname{MSE}}}
\newcommand{\loss}{{\mathcal{L}}}
\newcommand{\horizon}{{l}}

% Auto sized brackets
\DeclarePairedDelimiter\autobracket{(}{)}
\newcommand{\br}[1]{\autobracket*{#1}}

\DeclarePairedDelimiter\autobrackett{[}{]}
\newcommand{\brr}[1]{\autobrackett*{#1}}

\DeclarePairedDelimiter\autobrackettt{\{}{\}}
\newcommand{\brrr}[1]{\autobrackettt*{#1}}

\newcommand{\ssh}[1]{\textcolor{blue}{[#1--- ss]}}


%\newcommand*{\rom}[1]{\expandafter\@slowromancap\romannumeral #1@}
\newcommand{\rom}[1]{\uppercase\expandafter{\romannumeral #1\relax}}

